Closed Form Modelling and Identification of Banking Effects in Confined Waters

Vessels navigating in confined waters are subject to banking effects, which are hydrodynamic forces and moments arising from pressure differentials between the vessel sides, significantly affecting manoeuvrability and safety. Existing numerical approaches such as computational fluid dynamics (CFD) can accurately capture these effects but are computationally expensive and unsuitable for real-time control or estimation. This paper presents a closed-form, first-principles model of banking effects. The model coefficients are identified using physics-informed regression on towing tank experiment data for a scaled container vessel. Validation through Shapley value analysis confirms the significance of the banking terms in reproducing the measured forces and moments. Lastly, the derived coefficients are shown to be non-dimensional, making the model applicable across different scales that preserve vessel geometry.

==> sections/data.tex <==
\section{Data}
To verify the modelling approach, the coefficients for a towing model is determined from experiment data. The towing model is a 1:89.11 scale version of the Duisburg Test Case (DTC) vessel, which is a 14000 TEU Post-Panamax container ship model \cite{ElMoctar2012DuisburgBenchmarking}. The data used in this paper is from \cite{Eloot2016RunningPurposes} where harmonic yaw and sway captive tests, with constant forward velocity, were performed in a towing tank. Namely, two tests with harmonic yaw angle and zero sway (test A, B), and two tests with harmonic sway and zero rate of turn (test C, D), see \Cref{fig:traj_forces}. The forces and moments acting on the towing model are measured using a force-torque sensor mounted between the model and the towing rig.
\begin{figure}[ht]
    \centering
    %\textbf{Towing Experiment Data}\par\medskip
    \includegraphics[width=\linewidth]{figures/traj_forces.pdf}
    \caption{Model ship trajectories, forces, and moments for each test scenario, from \cite{Eloot2016RunningPurposes}.}
    \label{fig:traj_forces}
\end{figure}
\subsection{Dataset Partitioning}
The dataset must be split into a training and validation dataset. The data is split by randomly sampling 80 \% of the data for training and 20\% for validation, to ensure that both the training and validation data is sufficiently excited and to remove the temporal aspect of the data which will not be used in the modelling and estimation. 

\begin{comment}
The following collected data is of particular interest:
\begin{enumerate}
    \item Position $x$ and $y$ in canal (m)
    \item Heading $\psi$ in canal (rad)
    \item Surge velocity $u$ (m/s)
    \item Sway velocity $v$ (m/s)
    \item Rate of turn $r$ (rad/s)
    \item Surge acceleration $\dot{u}$
    \item Sway acceleration $\dot{v}$ (m/s$^2$)
    \item Angular acceleration $\dot{r}$ (rad/s$^2$)
    \item Sinkage $z$ (m)
    %\item Trim $\tau$
    \item Surge force $X$ (N)
    \item Sway force $Y$ (N)
    %\item Roll moment $K$
    \item Yaw moment $N$ (Nm)
\end{enumerate}
\end{comment}
